Self-assembling redox-wires form the 2D power grid of energy converting cell membranes

The light-driven reactions of photosynthesis, as well as the mitochondrial power supply, are hosted within specialized membranes containing a high fraction of redoxactive lipids. Protein mobility and diffusion of redox lipids is believed to be the in plane charge transfer mechanism along such cell membranes. Using a membrane-on-a-chip setup, we show that redox-active model membranes can conduct and sustain surprisingly high (mA) currents with a specific resistivity typical for semiconductors. Our data suggest that charge transfer within cell walls hosting electron-transferchains is driven by self-assembling molecular redox-wires that effectively couple redox-proteins by a simultaneous electron and proton in plane hopping within a membrane. This completely alters our understanding of the role of lipid membranes with wide-range implications suggesting e.g. that conducting membranes may be the precursor for evolving complex redox-machineries of life, and electrochemical membrane deterioration may play an important role in mitochondrial aging. Further, these self-assembling organic 2D-conductors offer technologically exploitable features allowing for designing self-assembling and adaptive bio-electronics.

==> __reply_to_referees.tex <==
% To DO:
% CV: 1 x gold chip, -0.1 +0.65 vs. Ag|AgCl, rates: 10 mV/s 100 mV/s 50 5 
% Test with large sheet electrode on LBT
% LBT: 20 mN mit 10%/20%/30% Q und 30% mit 15 20 30 mN/m
% Try pH indicator to vizualize... 



Reviewer 1: 
This is a beautiful paper and an eye-opener. The paper illustrates a new concept of 2D bioelectrochemical electron conduction along self-assembling, Q-enzyme containing lipid membranes. In their experiments, the authors clearly separate faradaic from capacitive contributions, thus proving validity of the concept. Not only that this concept may give completely new viewpoints on, e.g., cellular energy conversion, but it may also provide new ideas for biomimetic technologies and for bioelectronics. 
This is one of those papers that I would say: "Wish I had this idea!"
\textcolor{blue}
{

}

Reviewer 2: This manuscript reports a membrane-on-a-chip setup to measure in-plane conductivity and resistance of lipid bilayer membrane positioned in between two head-to-head electrodes. The authors selected a mixed membrane consisting of 30\% Q-enzymes as redox-active units and photospholipid DSPE as matrix, which was found to be able to conduct and sustain high current flow at the level of mA. They rationalized this behavior to be associated with in-plane simultaneous hopping of electron and proton along the self-assembled redox-active Q-enzyme wires, thus concluding that wiring up of redox units to form a kind of 2D structure is responsible of redox machinery of biological life. This work should have been an interesting study as it would help understand redox processes at/within membranes. 
However, I do not think this chemical system can mimic truly fluidic biological membranes, in which the charge transfer involves chain reactions between a variety of redox units in a 
We can assume that we have similarly fluid membranes to other SLBs in published literature.
\textcolor{blue}
{
%if a supported system would be a lower limit ---> membrane on a chip --> new approach to study this. 
}

"3D" confinement. 

The electron hopping can only occur among redox sites nanometer far away from each other, forming redox-wire like conductor to shuttle electron transfer seem to be unlikely. The authors need more data and in-depth analysis to prove the hypothesis. 
\textcolor{blue}
{%average distance is roughly 1 nm between two molecules (80 A^2/molecule), so it is a nanometer away and in accordance with e.g. redox polymers. This is now mentioned in the main text 
% average distance etc... 
}
Many details about experiment and data analysis were not clarified or included. The manuscript at its current stage does not merit publication by Angewandte Chemie.

Specific Comments:
1.	The paper is difficult to read as many abbreviations are not interpreted at their first appearance, for instances, "Q-membranes" and "DSPE". I am not able to fully catch their meaning if the reader has no expertise in the field or has to refer to supporting information. 
\textcolor{blue}
{Q-membranes is pretty clear given what the paper is about and we mention q-enzymes and quinones… DSPE is explained in supp. info, but should be explained in main body of text.
}
2.	Chemical structure shown in Figure 1a and that on the left side of Figure 1b are more appropriately named "phenols" instead of "quinones". 
\textcolor{blue}
{
Simply not correct: coenzyme q10 is literally called ubiquinone…
}
3.	The size/area of WE, CE1 is not given (only width = 5 mm was given). The authors did not describe CE2 either, electrode material, also gold? 

\textcolor{blue}
{WE area we should have said, CE-area is not relevant (and specified as pt wire in the supporting info, p1… might be we should have put that into the main text, don’t see how it undermines whether the results are believable).}


4.	The authors claimed the four-orders of magnitude higher current difference between Q-membrane and control is associated with Faradaic process. I would be curious to see the voltammetric signal (such as conventional cyclic voltammetry). In fact, this huge difference is abnormal since it means there is enormously huge amount of redox-active quinones. 
\textcolor{blue}
{I feel like voltammetry was done, if not this is something we should do.
}

5.	Actually, I do not really understand either why such an device was used with WE and RE separated by the membrane. Considering a high resistance of membrane in comparison with that of PBS-NaCl solutions, most likely major potential drop occur on the membrane instead of biasing on charge transfer. If possible, RE can be positioned on the same side by depositing solid-state Ag/AgCl on the chip?


\textcolor{blue}
{Unclear what is meant. Current transfer was not across membrane but along. Perhaps we could repeat the measurement with making sure the RE is as close as possible to WE.
}
6.	The authors fitted impedance data in Figure 3 to an circuit of 4 resistor-capacitor elements.Using CPE to represent capacitor is very tricky and details on fitting should be provided. Additionally, what does "coupled electron flow at lower frequencies" mean?
\textcolor{blue}
{
Using a CPE to represent imperfect capacitors is a very common practise. Not sure what further details he wants to see. However, we should probably clarify what coupled electron flow at low frequencies means.
}


Reviewer 3: 
The authors report a new approach based on a "membrane-on-a-chip" to investigate the charge transport in lipid bilayers containing a high fraction of quinones. These redox active units are linked to hydrophobic isoprenoid chains and incorporated in the bilayers. In other words, they should diffuse only in these model membranes and not in solution. The bilayers were deposited by the LB technique between two electrodes. The authors observed very high currents, up to 14 mA. Their interpretation is that the charge transport in the bilayer occurs by an electron-hopping process via electron-transfer chains formed by self-assembling molecular redox-wires.
The approach and the results are original and might be interesting and stimulating. But, considering the presented experimental results, I am not convinced by their interpretation. This study is incomplete and too preliminary. More control experiments are required as well as the SI is not detailed enough. In brief, my main concern is about the interpretation of the data (see below) and the lack of experimental data to support it. In addition, the authors over-interpret their results by claiming that they formed "self-assembling redox-wires". It is absolutely not demonstrated. Therefore, I recommend the rejection of this manuscript. 

Major points:
1)	The electron-hopping process is very well-known in electrochemistry and has been widely studied in redox polymer films for example. The charge diffusion in redox polymers involves an electron-hopping process from site to site where transport of both electrons and charge-compensating counter-ions occurs simultaneously. The distance between adjacent redox sites is the key factor governing the efficiency of the electron-transfer processes in the film and the rate of electron transfer decays exponentially with the distance between the redox centers in the transition state. In redox hydrogel films, electron-transferring collisions are effective when the distance between the oxidized and reduced redox centers is in the ~1−2 nm range. In addition, the mobility of the redox centers, which depends on the length of the flexible spacers is essential for the electron-hopping process. The authors should calculate the average distance between adjacent quinones to support their data. 

\textcolor{blue}
{Fair point. We should comment on what is known about electron hopping in polymers and compare our data analysis. We might also repeat experiments with different Q-concentrations to see if current changes.
%CV mit scan rates und Q concentrations
}
In addition, by changing the film compression by LB, they should observe very strong variations of the measured current because this will lead to a variation of the distance between adjacent redox sites. 

\textcolor{blue}
{
Not sure that film compression necessarily transfers to different lipid densities on the chip. I would guess that as the bilayer is fluid, it will always assume the same density more or less. We could do the experiment in the LB trough, though.
}
%repeat with CL --> 

2)	The measured currents (>mA) are very high for this configuration. The two gold electrodes (working and counter-electrodes) are separated by a 30 μm gap. But, I was not able to find the area of the electrodes. Depending on this parameter, the corresponding current density might be surprisingly high. This point should be specified and discussed. 
\textcolor{blue}
{
fair % Reply along back of the envelope: 0.7 mu/s - 1 Mio/Q/s --> switching limit bei ps/ Photosyn: 100% compare to this...
}

3)	The authors should study their system using cyclic voltammetry and vary the scan rate. It is essential to show the oxidation wave of the quinones, the surface confined features of the immobilized redox species, the dependence of the oxidation peak intensity with the scan rate, the electrochemical reversibility, etc. Considering the measured currents, cyclic voltammetric experiments could be easily performed and it will provide vital information to support the interpretation as the rate of electron transfer, if it occurs really in the membranes. 

\textcolor{blue}
{
as before, fair
}

4)	I am not convinced by the impedance measurements. This electrochemical characterization is not detailed enough because different equivalent circuits could be proposed for this system.
\textcolor{blue}
{

}

5)	It should be quite easy to image a pH gradient by microscopy at the level of the bilayers with a pH sensitive fluorescent probe. This would support the interpretation of the results.

\textcolor{blue}
{
fair. can we do it quickly? 
}

Minor points:
1)	The tile of the manuscript in the SI is different from the main text.
2)	In the SI, some figures are cited as "Figure ??".



==> old.tex <==
%Establishing of a transient grid is also obvious from the current transients shown in \texbf{Figure \ref{f2}} (see enlarged inset). 
%When a potential is established, first the local molecules on the electrodes are oxidized/reduced and the conducting grid is established, i.e. an increasingly higher current flow establishes over 10-20 seconds. The current peaks and slightly decays again by about (3\%). 
%In addition, the current never plateaus within the measured time frame, but indicates a shallow gradual slope towards smaller currents at prolonged current flow. 
%Here, the tendency to lower currents is likely due to establishing of a pH gradient, which can counteract the current flow with increasing time (see again \textbf{Figure \ref{f2}}). 
%In natural systems the pH gradient is compartmentalized, to further drive molecular engines of the respiratory chain, such as the ATP synthase, hence harvesting the proton chemical potential as well. 
%Here, we experimentally only utilize the electron cycle, the proton cycle must dissipate via the bulk electrolyte.  
